Enhancing Fine-grained Object Detection in Aerial Images via Orthogonal Mapping

Fine-Grained Object Detection (FGOD) is a critical task in high-resolution aerial image analysis. This letter introduces Orthogonal Mapping (OM), a simple yet effective method aimed at addressing the challenge of semantic confusion inherent in FGOD. OM introduces orthogonal constraints in the feature space by decoupling features from the last layer of the classification branch with a class-wise orthogonal vector basis. This effectively mitigates semantic confusion and enhances classification accuracy. Moreover, OM can be seamlessly integrated into mainstream object detectors. Extensive experiments conducted on three FGOD datasets (FAIR1M, ShipRSImageNet, and MAR20) demonstrate the effectiveness and superiority of the proposed approach. Notably, with just one line of code, OM achieves a 4.08% improvement in mean Average Precision (mAP) over FCOS on the ShipRSImageNet dataset. Codes are released at https://github.com/ZhuHaoranEIS/Orthogonal-FGOD.

==> fair1mv1.tex <==
% \begin{table}[t]
% \renewcommand{\arraystretch}{1.2}
% \caption{Comparison results on FAIR1M-v1.0 online validation}
% \centering
% \begin{tabular}{l c | c | c}%四个c代表该表一共四列，内容全部居中
% \toprule
% Method & Reference & Backbone & AP$_{0.5}$ \\
% \midrule
% \textit{one-stage methods:} \\ 
% \midrule
% RetinaNet~\cite{retinanet} & ICCV2017 & R-50-FPN  & 26.58  \\
% R3Det~\cite{r3det} & AAAI2021 & R-50-FPN  & 30.62  \\ % revise 30.6180
% S2ANet~\cite{s2anet} & TGRS2021 & R-50-FPN  & 34.71  \\ % revise 26.7095
% FCOS~\cite{fcos} & CVPR2019 & R-50-FPN  & 34.10  \\
% \midrule
% \textit{two-stage methods:} \\
% \midrule
% Faster R-CNN~\cite{faster-rcnn} & CVPR2018 & R-50-FPN  & 36.83  \\
% Oriented R-CNN~\cite{orcnn} & ICCV2021 & R-50-FPN  & 38.85  \\
% RoI Transformer~\cite{roitrans} & CVPR2019 & R-50-FPN  & 39.15  \\ 
% PETDet~\cite{petdet} & TGRS2023 & R-50-FPN  & 40.55  \\ 
% \midrule
% \textbf{FCOS w/OM} & ---- & R-50-FPN  &  \textbf{35.33}\\
% \textbf{PETDet w/OM} & ---- & R-50-FPN  & \textbf{41.19} \\
% \bottomrule
% \end{tabular}
% \label{table:fair1mv1}
% \end{table}

\begin{table}[t]
\renewcommand{\arraystretch}{1.2}
\caption{Comparison results on FAIR1M-v1.0 online validation.}
\centering
\begin{tabular}{l | c | c}%四个c代表该表一共四列，内容全部居中
\toprule
Method & Backbone & AP$_{0.5}$ \\
\midrule
\textit{one-stage methods:} \\ 
\midrule
RetinaNet~\cite{retinanet} & R-50-FPN  & 26.58  \\
R3Det~\cite{r3det} & R-50-FPN  & 30.62  \\ % revise 30.6180
S2ANet~\cite{s2anet} & R-50-FPN  & 34.71  \\ % revise 26.7095
FCOS~\cite{fcos} & R-50-FPN  & 34.10  \\
\midrule
\textit{two-stage methods:} \\
\midrule
Faster R-CNN~\cite{faster-rcnn} & R-50-FPN  & 36.83  \\
Oriented R-CNN~\cite{orcnn} & R-50-FPN  & 38.85  \\
RoI Transformer~\cite{roitrans} & R-50-FPN  & 39.15  \\ 
PETDet~\cite{petdet} & R-50-FPN  & 40.55  \\ 
\midrule
\textbf{FCOS w/OM} & R-50-FPN  &  \textbf{35.33}\\
\textbf{PETDet w/OM} & R-50-FPN  & \textbf{41.19} \\
\bottomrule
\end{tabular}
\label{table:fair1mv1}
\end{table}

==> fair1mv2.tex <==
% \begin{table}[t]
% \renewcommand{\arraystretch}{1.2}
% \caption{Comparison results on FAIR1M-v1.0 online validation}
% \centering
% \begin{tabular}{l c | c | c}%四个c代表该表一共四列，内容全部居中
% \toprule
% Method & Reference & Backbone & AP$_{0.5}$ \\
% \midrule
% \textit{one-stage methods:} \\ 
% \midrule
% RetinaNet~\cite{retinanet} & ICCV2017 & R-50-FPN  & 26.58  \\
% R3Det~\cite{r3det} & AAAI2021 & R-50-FPN  & 30.62  \\ % revise 30.6180
% S2ANet~\cite{s2anet} & TGRS2021 & R-50-FPN  & 34.71  \\ % revise 26.7095
% FCOS~\cite{fcos} & CVPR2019 & R-50-FPN  & 34.10  \\
% \midrule
% \textit{two-stage methods:} \\
% \midrule
% Faster R-CNN~\cite{faster-rcnn} & CVPR2018 & R-50-FPN  & 36.83  \\
% Oriented R-CNN~\cite{orcnn} & ICCV2021 & R-50-FPN  & 38.85  \\
% RoI Transformer~\cite{roitrans} & CVPR2019 & R-50-FPN  & 39.15  \\ 
% PETDet~\cite{petdet} & TGRS2023 & R-50-FPN  & 40.55  \\ 
% \midrule
% \textbf{FCOS w/OM} & ---- & R-50-FPN  &  \textbf{35.33}\\
% \textbf{PETDet w/OM} & ---- & R-50-FPN  & \textbf{41.19} \\
% \bottomrule
% \end{tabular}
% \label{table:fair1mv1}
% \end{table}

% \begin{table}[t]
% \renewcommand{\arraystretch}{1.2}
% \caption{Comparison results on FAIR1M-v2.0 online validation.}
% \centering
% \begin{tabular}{l | c | c}%四个c代表该表一共四列，内容全部居中
% \toprule
% Method & Backbone & AP$_{0.5}$ \\
% \midrule
% \multicolumn{3}{l}{\textit{one-stage methods:}} \\ 
% \midrule
% RetinaNet~\cite{retinanet} & R-50-FPN  & 26.07  \\
% S2ANet~\cite{s2anet} & R-50-FPN  & 30.93  \\ % revise 26.7095
% R3Det~\cite{r3det} & R-50-FPN  & 36.04  \\ % revise 30.6180
% FCOS~\cite{fcos} & R-50-FPN  & 39.37  \\
% \midrule
% \multicolumn{3}{l}{\textit{two-stage methods:}} \\
% \midrule
% Faster R-CNN~\cite{faster-rcnn} & R-50-FPN  & 41.64  \\
% Oriented R-CNN~\cite{orcnn} & R-50-FPN  & 43.90  \\
% RoI Transformer~\cite{roitrans} & R-50-FPN  & 44.03  \\ 
% PETDet~\cite{petdet} & R-50-FPN  & 44.93  \\ 
% \midrule
% \textbf{FCOS w/ OM} & R-50-FPN  &  \textbf{39.90}\\
% \textbf{PETDet w/ OM} & R-50-FPN  & \textbf{45.53} \\
% \bottomrule
% \end{tabular}
% \label{table:fair1mv2_short}
% \end{table}

\begin{table}[t]
\renewcommand{\arraystretch}{1.2}
\caption{Comparison results on FAIR1M-v2.0 online validation.}
\centering
\begin{tabular}{l | c | c}%四个c代表该表一共四列，内容全部居中
\toprule
Method & Backbone & AP$_{0.5}$ \\
\midrule
\multicolumn{3}{l}{\textit{one-stage methods:}} \\ 
\midrule
RetinaNet~\cite{retinanet} & R-50-FPN  & 26.07  \\
S2ANet~\cite{s2anet} & R-50-FPN  & 30.93  \\ % revise 26.7095
R3Det~\cite{r3det} & R-50-FPN  & 36.04  \\ % revise 30.6180
FCOS~\cite{fcos} & R-50-FPN  & 39.37  \\
% \midrule
FCOS w/ OM & R-50-FPN  &  \textbf{39.90}\\
\midrule
\multicolumn{3}{l}{\textit{two-stage methods:}} \\
\midrule
Faster R-CNN~\cite{faster-rcnn} & R-50-FPN  & 41.64  \\
Oriented R-CNN~\cite{orcnn} & R-50-FPN  & 43.90  \\
RoI Transformer~\cite{roitrans} & R-50-FPN  & 44.03  \\ 
PETDet~\cite{petdet} & R-50-FPN  & 44.93  \\ 
% \midrule
PETDet w/ OM & R-50-FPN  & \textbf{45.53} \\
\bottomrule
\end{tabular}
\label{table:fair1mv2_short}
\end{table}

==> fair1mv2_detail.tex <==
% \begin{table*}[t]
% \renewcommand{\arraystretch}{1.1}
% \caption{Comparison results on FAIR1M-2.0 online validation}
% \centering
% % \rowcolors{1}{green!40}{white}
% \begin{tabular}{c | c | c c c c c c c c | c c}%四个c代表该表一共四列，内容全部居中
% \toprule
% \multicolumn{2}{c}{Method} & RetinaNet~\cite{retinanet} & S2ANet~\cite{s2anet} & R3Det~\cite{r3det} & FCOS~\cite{fcos} & FRCNN~\cite{faster-rcnn} & ORCNN~\cite{orcnn} & RoI Trans~\cite{roitrans} & PETDet~\cite{petdet} & \textbf{FCOS w/OM} &  \textbf{PETDet w/OM} \\
% \midrule
% \multicolumn{2}{c}{Backbone} & R-50 & R-50 & R-50 & R-50 & R-50 & R-50 & R-50 & R-50 & R-50 & R-50 \\
% \midrule
% \multirow{10}{*}{Airplane} & B737 & 37.60 & 39.74 & 39.28 & 39.53 & 42.29 & 44.16 & 46.52 & 46.12 & 41.74 & 50.43 \\
%  & B747 & 86.54 & 88.74 & 87.47 & 92.64 & 92.73 & 93.13 & 93.05 & 93.40 & 92.80 & 93.90 \\
%  & B777 & 28.21 & 33.51 & 31.33 & 35.81 & 35.68 & 39.64 & 41.60 & 42.53 & 36.07 & 45.90 \\
%  & B787 & 48.91 & 52.09 & 53.93 & 58.96 & 60.36 & 61.41 & 62.88 & 66.52 & 58.40 & 63.41 \\
%  & C919 & 0.44  & 0.50  & 0.70  & 1.04  & 8.90  & 2.25  & 9.90  & 22.32 & 7.61 & 30.20 \\
%  & A220 & 51.19 & 49.34 & 51.77 & 54.09 & 54.03 & 54.53 & 53.80 & 56.86 & 55.29 & 58.22 \\
%  & A321 & 65.89 & 70.52 & 69.87 & 69.54 & 68.34 & 70.61 & 71.07 & 73.66 & 70.28 & 73.81 \\
%  & A330 & 27.86 & 47.54 & 44.99 & 57.06 & 58.69 & 59.94 & 61.48 & 62.79 & 55.75 & 64.83 \\
%  & A350 & 50.82 & 47.07 & 55.16 & 64.91 & 67.67 & 67.54 & 67.02 & 69.08 & 67.70 & 73.29 \\
%  & ARJ21& 3.47  & 2.20  & 2.75  & 6.27  & 9.97  & 11.97 & 14.35 & 10.35 & 6.11  & 18.29 \\
%  \midrule
% \multirow{8}{*}{Ship} & PS & 1.92 & 4.80 & 9.62 & 11.66 & 12.00 & 15.20 & 12.71 & 13.12 & 12.75 & 12.31 \\
%  & MB  & 10.74 & 23.47 & 38.26 & 52.58 & 53.17 & 59.62 & 58.74 & 61.93 & 52.34 & 60.95 \\
%  & FB  & 1.43  & 4.67  & 9.55  & 14.86 & 16.99 & 26.46 & 19.33 & 21.95 & 12.76 & 19.84 \\
%  & TB  & 12.87 & 15.62 & 25.39 & 29.38 & 29.38 & 30.23 & 30.79 & 29.59 & 29.83 & 29.53 \\
%  & ES  & 4.32  & 7.59  & 10.44 & 14.42 & 13.00 & 15.92 & 13.81 & 17.37 & 15.98 & 16.78 \\
%  & LCS & 8.33  & 31.81 & 46.48 & 46.42 & 43.29 & 49.06 & 46.96 & 47.66 & 46.91 & 50.50 \\
%  & DCS & 14.11 & 33.34 & 45.84 & 48.20 & 44.45 & 51.12 & 50.52 & 49.36 & 47.79 & 48.86 \\
%  & WS  & 1.21  & 7.16  & 22.32 & 29.27 & 20.27 & 32.37 & 27.33 & 30.46 & 28.25 & 30.48 \\
%  \midrule

% \multirow{9}{*}{Vehicle} & SC & 30.40 & 47.77 & 51.17 & 52.09 & 53.78 & 56.87 & 58.10 & 68.74 & 51.80 & 68.75 \\
%  & BUS & 2.69  & 2.38  & 3.95  & 13.96 & 25.68 & 30.46 & 31.76 & 33.64 & 19.43 & 33.91 \\
%  & CT  & 8.49  & 19.75 & 34.27 & 40.92 & 47.36 & 49.95 & 49.76 & 51.74 & 42.07 & 51.50 \\
%  & DT  & 10.09 & 24.10 & 27.98 & 28.79 & 45.69 & 48.82 & 48.78 & 48.98 & 29.55 & 48.40 \\
%  & VAN & 20.81 & 39.53 & 43.50 & 47.74 & 47.87 & 51.39 & 52.92 & 65.45 & 47.55 & 65.72 \\
%  & TRI & 0.00  & 0.08  & 10.43 & 11.81 & 12.17 & 15.99 & 13.68 & 11.64 & 10.89 & 10.77 \\
%  & TRC & 0.00  & 0.08  & 0.26  & 0.96  & 1.58  & 1.85  & 1.81  & 0.00  & 0.81  & 0.36 \\
%  & EX  & 0.16  & 1.71  & 4.84  & 9.43  & 11.15 & 15.26 & 13.21 & 8.49  & 9.24  & 9.55  \\
%  & TT  & 0.00  & 0.02  & 0.42  & 3.94  & 13.45 & 5.39  & 16.34 & 9.12  & 11.54 & 8.56  \\
%  \midrule

% \multirow{4}{*}{Court} & BC & 30.54 & 40.69 & 47.66 & 48.49 & 55.38 & 57.56 & 56.90 & 49.85 & 42.42 & 48.53 \\
%  & TC & 74.59 & 79.13 & 85.68 & 86.56 & 88.40 & 88.56 & 88.88 & 86.05 & 86.15 & 86.40 \\
%  & FF & 54.73 & 46.33 & 59.33 & 57.50 & 60.23 & 63.34 & 62.80 & 64.69 & 56.26 & 64.87 \\
%  & BF & 87.28 & 87.14 & 90.25 & 89.02 & 91.47 & 90.90 & 90.81 & 90.79 & 89.08 & 91.14 \\
%  \midrule

% \multirow{3}{*}{Road} & IS & 60.07 & 56.07 & 61.23 & 62.82 & 65.04 & 64.57 & 64.40 & 61.55 & 63.15 & 62.97 \\
%  & RA & 35.13 & 29.15 & 33.17 & 31.34 & 33.09 & 31.24 & 31.90 & 31.61 & 30.59 & 29.24 \\
%  & BR & 15.46 & 18.02 & 25.97 & 26.60 & 32.18 & 35.36 & 32.99 & 26.69 & 27.53 & 25.67 \\
%  \midrule

% \multicolumn{2}{c}{$AP_{50}$} & 26.07 & 30.93 & 36.04 & 39.37 & 41.64 & 43.90 & 44.03 & 44.83 & 39.90 & \textbf{45.53} \\
% \bottomrule
% \end{tabular}
% \end{table*}

\begin{table*}[t]
\renewcommand{\arraystretch}{1.1}
\caption{Comparison results on FAIR1M-v2.0 online validation. All the models are with ResNet-50 as the backbone. Moreover, FRCNN, ORCNN, and RoI Trans denote Faster R-CNN, Oriented R-CNN and RoI Transformer respectively.}
\centering
% \rowcolors{1}{green!40}{white}
\begin{tabular}{c | c | c c c c c c | c c}%四个c代表该表一共四列，内容全部居中
\toprule
\multicolumn{2}{c}{Method}  & S2ANet~\cite{s2anet}  & FCOS~\cite{fcos} & FRCNN~\cite{faster-rcnn} & ORCNN~\cite{orcnn} & RoI Trans~\cite{roitrans} & PETDet~\cite{petdet} & \textbf{FCOS w/OM} &  \textbf{PETDet w/OM} \\
\midrule
\multicolumn{2}{c}{Backbone} & R-50 & R-50 & R-50 & R-50 & R-50 & R-50 & R-50 & R-50 \\
\midrule
\multirow{10}{*}{Airplane} & B737 & 39.74 & 39.53 & 42.29 & 44.16 & 46.52 & 46.12 & 41.74 & 50.43 \\
 & B747 & 88.74 & 92.64 & 92.73 & 93.13 & 93.05 & 93.40 & 92.80 & 93.90 \\
 & B777 & 33.51 & 35.81 & 35.68 & 39.64 & 41.60 & 42.53 & 36.07 & 45.90 \\
 & B787 & 52.09 & 58.96 & 60.36 & 61.41 & 62.88 & 66.52 & 58.40 & 63.41 \\
 & C919 & 0.50  & 1.04  & 8.90  & 2.25  & 9.90  & 22.32 & 7.61 & 30.20 \\
 & A220 & 49.34 & 54.09 & 54.03 & 54.53 & 53.80 & 56.86 & 55.29 & 58.22 \\
 & A321 & 70.52 & 69.54 & 68.34 & 70.61 & 71.07 & 73.66 & 70.28 & 73.81 \\
 & A330 & 47.54 & 57.06 & 58.69 & 59.94 & 61.48 & 62.79 & 55.75 & 64.83 \\
 & A350 & 47.07 & 64.91 & 67.67 & 67.54 & 67.02 & 69.08 & 67.70 & 73.29 \\
 & ARJ21& 2.20  & 6.27  & 9.97  & 11.97 & 14.35 & 10.35 & 6.11  & 18.29 \\
 \midrule
\multirow{8}{*}{Ship} & PS & 4.80 & 11.66 & 12.00 & 15.20 & 12.71 & 13.12 & 12.75 & 12.31 \\
 & MB  & 23.47 & 52.58 & 53.17 & 59.62 & 58.74 & 61.93 & 52.34 & 60.95 \\
 & FB  & 4.67  & 14.86 & 16.99 & 26.46 & 19.33 & 21.95 & 12.76 & 19.84 \\
 & TB  & 15.62 & 29.38 & 29.38 & 30.23 & 30.79 & 29.59 & 29.83 & 29.53 \\
 & ES  & 7.59  & 14.42 & 13.00 & 15.92 & 13.81 & 17.37 & 15.98 & 16.78 \\
 & LCS & 31.81 & 46.42 & 43.29 & 49.06 & 46.96 & 47.66 & 46.91 & 50.50 \\
 & DCS & 33.34 & 48.20 & 44.45 & 51.12 & 50.52 & 49.36 & 47.79 & 48.86 \\
 & WS  & 7.16  & 29.27 & 20.27 & 32.37 & 27.33 & 30.46 & 28.25 & 30.48 \\
 \midrule

\multirow{9}{*}{Vehicle} & SC & 47.77 & 52.09 & 53.78 & 56.87 & 58.10 & 68.74 & 51.80 & 68.75 \\
 & BUS & 2.38  & 13.96 & 25.68 & 30.46 & 31.76 & 33.64 & 19.43 & 33.91 \\
 & CT  & 19.75 & 40.92 & 47.36 & 49.95 & 49.76 & 51.74 & 42.07 & 51.50 \\
 & DT  & 24.10 & 28.79 & 45.69 & 48.82 & 48.78 & 48.98 & 29.55 & 48.40 \\
 & VAN & 39.53 & 47.74 & 47.87 & 51.39 & 52.92 & 65.45 & 47.55 & 65.72 \\
 & TRI & 0.08  & 11.81 & 12.17 & 15.99 & 13.68 & 11.64 & 10.89 & 10.77 \\
 & TRC & 0.08  & 0.96  & 1.58  & 1.85  & 1.81  & 0.00  & 0.81  & 0.36 \\
 & EX  & 1.71  & 9.43  & 11.15 & 15.26 & 13.21 & 8.49  & 9.24  & 9.55  \\
 & TT  & 0.02  & 3.94  & 13.45 & 5.39  & 16.34 & 9.12  & 11.54 & 8.56  \\
 \midrule

\multirow{4}{*}{Court} & BC & 40.69 & 48.49 & 55.38 & 57.56 & 56.90 & 49.85 & 42.42 & 48.53 \\
 & TC & 79.13 & 86.56 & 88.40 & 88.56 & 88.88 & 86.05 & 86.15 & 86.40 \\
 & FF & 46.33 & 57.50 & 60.23 & 63.34 & 62.80 & 64.69 & 56.26 & 64.87 \\
 & BF & 87.14 & 89.02 & 91.47 & 90.90 & 90.81 & 90.79 & 89.08 & 91.14 \\
 \midrule

\multirow{3}{*}{Road} & IS & 56.07 & 62.82 & 65.04 & 64.57 & 64.40 & 61.55 & 63.15 & 62.97 \\
 & RA & 29.15 & 31.34 & 33.09 & 31.24 & 31.90 & 31.61 & 30.59 & 29.24 \\
 & BR & 18.02 & 26.60 & 32.18 & 35.36 & 32.99 & 26.69 & 27.53 & 25.67 \\
 \midrule

\multicolumn{2}{c}{AP$_{0.5}$} & 30.93 & 39.37 & 41.64 & 43.90 & 44.03 & 44.83 & \textbf{39.90} & \textbf{45.53} \\
\bottomrule
\end{tabular}
\label{table:fair1mv2}
\end{table*}

==> pseudocode.tex <==
\begin{algorithm}[t] 
\caption{ Orthogonal Mapping.} 
\label{alg:OM code} 
\begin{algorithmic}[1] %这个1 表示每一行都显示数字
\REQUIRE ~~\\ %算法的输入参数：Input
The input feature tensor $X$, $X \in \mathbb{R}^{N \times H \times W}$\\
The convolution kernel $K$, $K \in \mathbb{R}^{C \times k \times k \times N}$ 
\ENSURE ~~\\ %算法的输出：Output
The classification confidence $Y$, $Y \in  \mathbb{R}^{H \times W \times C}$
\STATE random initialization
\STATE \colorbox{gray!20}{\quad \qquad \qquad \qquad /* previous method*/ \qquad \qquad \qquad \ }
\STATE \colorbox{gray!20}{$Y = Conv(K, X)$; \quad \quad \quad
 \qquad \qquad \qquad\qquad\qquad \ \ \! \ } 
 \STATE \colorbox{yellow!20}{\qquad \qquad \qquad \qquad /* our method*/ \qquad \qquad \qquad \quad \ }
 \STATE \colorbox{yellow!20}{$K = AvgPooling(K), K \in \mathbb{R}^{C \times 1 \times 1 \times N}$;  \qquad \qquad \quad } 
\STATE \colorbox{yellow!20}{$K = flatten(K), K \in \mathbb{R}^{C \times N}$; \qquad \qquad \qquad \qquad \quad } 
\STATE \colorbox{yellow!20}{$\tilde{K} = Gram\_Schmidt(K)$; \quad \quad \quad \quad  \quad \quad \quad \quad \ \ \qquad  } 
\STATE \colorbox{yellow!20}{$Y = {\langle \tilde{K}, X \rangle}^T$;\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad  \quad \quad \quad \quad \qquad } 

% \colorbox{gray!10}{This line has a background color}
\RETURN $Y$; %算法的返回值
\end{algorithmic}
\end{algorithm}
